Leveraging Structured Information for Explainable Multi-hop Question Answering and Reasoning

Neural models, including large language models (LLMs), achieve superior performance on multi-hop question-answering. To elicit reasoning capabilities from LLMs, recent works propose using the chain-of-thought (CoT) mechanism to generate both the reasoning chain and the answer, which enhances the model's capabilities in conducting multi-hop reasoning. However, several challenges still remain: such as struggling with inaccurate reasoning, hallucinations, and lack of interpretability. On the other hand, information extraction (IE) identifies entities, relations, and events grounded to the text. The extracted structured information can be easily interpreted by humans and machines (Grishman, 2019). In this work, we investigate constructing and leveraging extracted semantic structures (graphs) for multi-hop question answering, especially the reasoning process. Empirical results and human evaluations show that our framework: generates more faithful reasoning chains and substantially improves the QA performance on two benchmark datasets. Moreover, the extracted structures themselves naturally provide grounded explanations that are preferred by humans, as compared to the generated reasoning chains and saliency-based explanations.

==> 2_method_old.tex <==
\section{Methodology}

%\xd{``Methodology'', experiments should be the next section}

In this section, we firstly give a formal introduction of the multi-hop question answering task.
We then provide definitions of elements in the semantic graphs that are to be extracted and utilized in the QA framework.
Third, we introduce our specific prompting based methods based on the graphs.
% nodes and relations in graphs
% and propose graph structures. 
% Graphs are finally represented in text format.

\subsection{Task}
Given a question, and several candidate paragraphs, we aim to obtain the answers that involve multi-hop reasoning.
We tackle the task with in-context learning from two different settings: 
(1) directly generate the answer from the context and question, namely (``\textit{few-shot setting}'');
(2) generate the answer as well as the explanations. -- one representative method aiming is chain-of-thought reasoning (CoT)~\cite{weichain}. We name is ``\textit{CoT}'' setting here.
\xd{to add more}

\subsection{Elements of Semantic Structures (Graphs)}

[formulate all definitions]

To build a graph that is simple to represent and includes the most useful information in a text sequence, the definition of nodes and edges is essential.

Nodes and edges are basic elements in a graph. To convert a text sequence to a graph, entities are widely seen as nodes, and semantic relations are commonly seen as edges. Many methods exist to extract them from sentences, such as entity recognition and relation extraction.

Named entity recognition (NER) is widely used to extract and classify text spans in an unstructured sequence into pre-defined categories. Most extracted named entities are real-world objects, such as persons, organizations, time, locations, etc. They can present objectives in good form. However, they are not enough to represent a paragraph. One main reason is that those categories can hardly present events.

In our work, we define a node as a short text sequence that completely represents a role in the whole sentence.

[example]

Relations are categorized as closed relations and open relations. Closed relations are pre-defined and manually defined. For example, Wikidata has 11,008 properties (relations). Each property is proposed and fully discussed by people before publishing. Thus, the number of closed relations is limited. They can hardly be used to present complex relations between entities that are defined above. Open relations are hard to define due to the complex relations between entities.

In our work, we define an edge as a short text sequence representing semantic relations between two entities.

[example]

% The semantic roles labeling (SRL) method converts a text sequence to a structure. But, 

\subsection{Constructing Graphs with Prompting}

We proposed two different graphs: the entity-only graph and the entity-relation graph. Both of them are generated by a large language model.
%\xd{don't specify which specific model is used here, using ``one LLM(s)'' instead. Details like this should be put in the experimental results section}. 
For both graph generations, we add demonstrations at the beginning for the model to refer to. Also, the graph generation process includes two steps: entity generation and graph generation.

\paragraph{Entity and Relation Extraction}
The demonstration for the entity generation step includes two parts: a document and a list of entities. The part of the document includes a sample Wikipedia paragraph. It has the word "Document:" as a start as the indication. Then, it is followed by a paragraph with a title. The entity part starts with the "Entities:". Then, all entities are listed line-by-line. Overall, it looks like:
{\ttfamily
\begin{align*}
\small \raggedleft
% \fontfamily{helvet}\selectfont 
& \text{Document:} \\
& \text{Wikipedia Title: <Page Title>} \\
& \text{<Paragraph Text>} \\
\\
& \text{Entities: } \\
& \text{<Entity 1>} \\
& \text{<Entity 2>} \\
& \text{...} \\
& \text{<Entity n>}
\end{align*}
}

The prompt template for the current paragraph is almost the same as above except for all <Entity x>.

\paragraph{Graph generation (KG1)}
\xd{to add a Fig demonstrating KG1 (all connected) and KG2 (with semantic relations)}
The entity-only graph and entity-relation graph are different at the graph generation step. For entity-only graphs, it is a pack of all entities. The graph looks like the following:
\begin{align*}
(<Entity 1>, <Entity 2>, \cdots,  <Entity n>)
\end{align*}

%% wondering whether this explanation is necessary, or they should be mentioned in the appendix
Since all entities in a paragraph may have relations between them, all entities should have relations with each other. A straightforward graph is a $N^2$ full graph in which each pair of entities has a pair to represent their relationship. The graph looks like this:
\begin{align*}
\small
& \text{(<Entity 1>, <Entity 2>)} \\
& \text{(<Entity 1>, <Entity 3>)} \\
& \cdots \\
& \text{(<Entity n-1>, <Entity n>)}
\end{align*}
However, this structure has so many disadvantages. Firstly, it is too long for model inputs. Then, information is redundant. Thus, after generating all entities, we pack all entities in a paragraph into a list.

\paragraph{Graph generation (KG2)}
The entity-relation graph contains both entities and relations. Besides all parts in the prompt template for the demonstration of the entity generation step, the demonstration of the entity generation step has another component: the sample graph. It is composed of a list of triples. Each triple includes a subject, a relation, and an object. The prompt template for its demonstrations looks like the following:
\begin{align*}
\small
& \text{Document:} \\
& \text{Wikipedia Title: <Page Title>} \\
& \text{<Paragraph Text>} \\
\\
& \text{Entities: } \\
& \text{<Entity 1>} \\
& \text{<Entity 2>} \\
& \cdots \\
& \text{<Entity n>} \\
\\
& \text{Graph:} \\
& \text{(<Entity 1>, <Relation 1>, <Entity x>)} \\
& \text{(<Entity 1>, <Relation 2>, <Entity y>)} \\
& \cdots \\
& \text{(<Entity i>, <Relation j>, <Entity z>)}
\end{align*}
The prompt template for the current paragraph is almost the same as above except for all lines after "Graph:".

In this graph structure, not all pairs of entities have relations. The LLM will generate relations for all pairs of entities if it exists.

\paragraph{Graph generation (KG2-D)}

Besides generating entity-relation graphs step-by-step, they can be generated directly by the language model. By giving graph demonstrations directly, the large language model can generate triples from given documents. The demonstration is composed of two parts: a document and a graph. The prompt template looks like the following:

\begin{align*}
\small
& \text{Document:} \\
& \text{Wikipedia Title: <Page Title>} \\
& \text{<Paragraph Text>} \\
\\
& \text{Graph:} \\
& \text{(<Entity 1>, <Relation 1>, <Entity x>)} \\
& \text{(<Entity 1>, <Relation 2>, <Entity y>)} \\
& \cdots \\
& \text{(<Entity i>, <Relation j>, <Entity z>)}
\end{align*}

The prompt template for the current paragraph is almost the same as above except for all lines after "Graph:".

\subsection{Overall Strucutre}

For each question, we currently have golden paragraphs. For each paragraph, a graph is generated as described above. Then, all documents and graphs are combined together to form the overall prompt template. Thus, the overall prompt template includes three components: documents, a graph, and a question prompt.

The documents part starts with "Documents:" and is followed by multiple graphs with titles. The graph part starts with "Graph:". All corresponding graphs are vertically concatenated. The following prompt is for the question. If the answer part includes a reasoning chain before the final answer, a question prompt, "Answer the following question by reasoning step-by-step," is added ahead of the real question, as described in the paper [cite harsh]. Otherwise, this part only contains a question, and the question prompt is empty.

\begin{align*}
\small
& \text{Documents:} \\
& \text{Wikipedia Title: <Page Title>} \\
& \text{<Paragraph Text>} \\
& \cdots \\
& \text{Wikipedia Title: <Page Title>} \\
& \text{<Paragraph Text>} \\
\\
& \text{Graph:} \\
& \text{<graph 1>} \\
& \cdots \\
& \text{<graph n>} \\
\\
& \text{Q: <question prompt> <question>} \\
& \text{A: }
\end{align*}

\subsection{Reasoning Chain}

In this task, we define reasoning chains as a list of short sentences in the right logical order. Each sentence only represents a relation between two entities. The last sentence is fixed to the format: "So the answer is: <answer>". The format of the last sentence is from [cite harsh's paper]. This helps clearly display reasoning chains and match the format of the graph. Also, it helps extract answers automatically from reasoning chains. In demonstrations, we provide reasoning chains in this format for reference if reasoning chains are requested.
Moreover, we apply a regex expression to extract answers from reasoning chains after it is generated.




==> tables/error_types.tex <==
\begin{table}[t]
\centering
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc}
\toprule
Error Type                            & Base prompt  & KG1 P. &  KG2 P. \\ \midrule
cannot understand documents & 46.43\% & 50.00\%          & 30.30\%          \\
Incomplete graph / poor graph quality & -       & -                & 15.15\%          \\
needs extra common sense knowledge    & 3.57\%  & 4.17\%           & 6.06\%           \\
over-reasoned                         & 14.29\% & 4.17\%           & -                \\
unanswerable                          & 35.71\% & 41.67\%          & 33.33\%          \\
others                                & -       & -           & 15.15\%          \\ \midrule
Grand Total \#Errors                          & 28      & 24               & 33              \\
\bottomrule
\end{tabular}
}
    \caption{Error made by different approaches on the 2WikiMultiHopQA test examples.}
    \label{tab:error_analysis_2wiki}
\end{table}
